Suppression of decoherence dynamics by a dissipative bath at strong coupling

Control of decoherence in open quantum systems has become a topic of great interest due to the emergence of quantum technologies that depend on quantum coherent effects. In this work, we investigate the decoherence dynamics of systems coupled to multiple baths through noncommuting systems' operators, and beyond the weak system-bath coupling limit. By building on cooperative effects between baths, we propose a novel strategy to mitigate rapid decoherence. Concretely, we study the dynamics of a qubit coupled to multiple environments with arbitrary interaction strengths, and along different coordinates. Based on insights gained on the decoherence dynamics from the analytical Effective Hamiltonian method, we carry out numerical simulations using the Reaction Coordinate quantum master equation method. In contrast to standard expectations, we show that when the system strongly interacts with a decohering bath, increasing its coupling to a second, dissipative bath slows down the decoherence dynamics. Our work offers insights into the preservation of quantum coherences in open quantum systems based on frustration effects, by utilizing cooperative effects between different heat baths.

==> editor.tex <==

Dear Editor:

We would like to submit to Physical Review A our manuscript: "Suppression of decoherence dynamics by a dissipative bath at strong coupling" by Jitian Chen, Jakub Garwola, and Dvira Segal.

In this work, we describe a counterintuitive approach to suppress the decoherence dynamics of a qubit coupled to multiple heat baths. 
Building on strong coupling effects, we show that extremely fast decohernece rates can be slowed down when the qubit is made to couple to a second dissipative bath.
This effect arises for the combination of strong coupling physics with the non-cummutativity of the system coupling operators to the baths. Our results are established through both an analytic approach and numerical simulations thus providing both intuition and accurate numerical results.

Recent studies discovered the unique effect of increasing the qubit lifetime during readout [60].  Our work contributes to this effort of understanding how multiple environments impact the population and coherence lifetimes of qubits.

We believe that our work will be of a significant interest to a broad community interested in open quantum systems for quantum information, light-matter systems and their control, and quantum material's engineering. 

Thank you for your consideration,
Jitian Chen, Jakub Garwola and Dvira Segal

Suggested Referees

Archana Kamal; Northwestern 

Camile Latune, Université de Bourgogne, France

Janet Anders, Exeter

Yoshitaka Tanimura, Kyoto University

Neill Lambert, Senior Research Scientist, RIKEN

Jonathan Keeling,  St Andrews University
